Zeroes of polynomials on definable hypersurfaces: pathologies exist, but they are rare

Given a sequence $\{Z_d\}_{d\in \mathbb{N}}$ of smooth and compact hypersurfaces in $\mathbb{R}^{n-1}$, we prove that (up to extracting subsequences) there exists a regular definable hypersurface $\Gamma\subset \mathbb{R}\mathrm{P}^n$ such that each manifold $Z_d$ appears as a component of the zero set on $\Gamma$ of some polynomial of degree $d$. (This is in sharp contrast with the case when $\Gamma$ is algebraic, where for example the homological complexity of the zero set of a polynomial $p$ on $\Gamma$ is bounded by a polynomial in $\mathrm{deg}(p)$.) We call these "pathological examples". In particular, we show that for every $0 \leq k \leq n-2$ and every sequence of natural numbers $a=\{a_d\}_{d\in \mathbb{N}}$ there is a regular, compact and definable hypersurface $\Gamma\subset \mathbb{R}\mathrm{P}^n$, a subsequence $\{a_{d_m}\}_{m\in \mathbb{N}}$ and homogeneous polynomials $\{p_{m}\}_{m\in \mathbb{N}}$ of degree $\mathrm{deg}(p_m)=d_m$ such that: \begin{equation} \label{eq:pathintro} b_k(\Gamma\cap Z(p_m))\geq a_{d_m}.\end{equation} (Here $b_k$ denotes the $k$-th Betti number.) This generalizes a result of Gwo\'zdziewicz, Kurdyka and Parusi\'nski. On the other hand, for a given definable $\Gamma$ we show that the Fubini-Study measure, in the gaussian space of polynomials of degree $d$, of the set $\Sigma_{d_m,a, \Gamma}$ of polynomials verifying $b_k(\Gamma\cap Z(p_m))\geq a_{d_m}$ is positive, but there exists a contant $c_\Gamma$ such that this measure can be bounded by: \begin{equation} 0<\mathbb{P}(\Sigma_{d_m, a, \Gamma})\leq \frac{c_{\Gamma} d_m^{\frac{n-1}{2}}}{a_{d_m}}. \end{equation} This shows that the set of "pathological examples" has "small" measure.

==> motivation.tex <==
Results of this type are basic building blocks in recent advances in incidence
problems in the area of discrete geometry driven by the polynomial partitioning
method \cite{Guth-Katz, Solymosi-Tao}. Recently, using different techniques
such incidence results have
been generalized from the semi-algebraic case to more general situations --
namely, incidences between definable sets over arbitrary o-minimal expansions of
$\mathb{R}$ (\cite{Basu-Raz, Galvin-Chernikov-Starchenko}. (We refer the reader
who is unfamiliar with o-minimal gemoetry) to \cite{Dries,Michel2} for easy to read introduction to the topic.) 
In order to
extend the polynomial partitioning technique to th eo-minimal situation
(as noted in \cite{OWF-report})
it is important to study the function $\beta_{\Gamma,0}$
where $\Gamma$ is now an arbitrary definable curve in an o-minimal structure
(rather than just semi-algebraic).
Unfortunately, in general nothing can be said about its behavior. For instance, ...



